Field Theoretic Study of Bilayer Membrane Fusion III: Membranes with Leaves of Different Composition

We extend previous work on homogeneous bilayers to calculate the barriers to fusion of planar bilayers which contain two different amphiphiles, a lamellae-former and a hexagonal former, with different compositions of the twoin each leaf. Self-consistent field theory is employed, and both standard and alternative pathways are explored. We first calculate these barriers as the amount of hexagonal former is increased equally in both leaves to levels appropriate to the plasma membrane of human red blood cells. We follow these barriers as the composition of hexagonal-formers is then increased in the cis layer and decreased in the trans layer, again to an extent comparable to the biological system. We find that, while the fusion pathway exhibits two barriers in both the standard and alternative pathways, in both cases the magnitudes of these barriers are comparable to one another, and small, on the order of 13 kT. As a consequence, one expects that once the bilayers are brought sufficiently close to one another to initiate the process, fusion should occur rapidly.

==> kkfusion06 <==

@Article{Bailey94,
  author = {A. L. Bailey and P. R. Cullis},
  title = {Modulation of membrane fusion by assymmetric transbilayer 
          distributions of amino lipids},
  journal = {Biochemistry},
  year = {1994},
  volume = {33},
  pages = {12573-12580}
} 


@Article{Bates99,
  author = 	 {F.S. Bates and G.H. Fredrickson},
  title = 	 {Block copolymers-designer soft materials},
  journal = 	 {Physics Today},
  year = 	 {1999},
  volume = 	 {52},
  pages = 	 {32-38}
}

@Article{Bonnafous00,
  author = 	 {P. Bonnafous and  T. Stegmann},
  title = 	 {Membrane perturbation and fusion pore formation in 
influenza hemagglutinin-mediated membrane fusion},
  journal = 	 {J. Biol. Chem.},
  year = 	 {2000},
  volume = 	 {275},
  pages = 	 {6160-6166}
}

@Article{Blumenthal03,
  author = 	 {R. Blumenthal and M. J. Clague and S.R. Durell and R.M. Epand},
  title = 	 {Membrane fusion},
  journal = 	 {Chem. Rev.},
  year = 	 {2003},
  volume = 	 {103},
  pages = 	 {53-69}
}

@Article{Carmesin88,
  author = 	 {I. Carmesin and K. Kremer},
  title = 	 {The bond fluctuation method: a new effective algorithm for the dynamics of polymers in all spatial dimensions.},
  journal = 	 {Macromolecules},
  year = 	 {1988},
  volume = 	 {21},
  pages = 	 {819-2823}
}


@Article{Cevc99,
  author = 	 {G. Cevc and H. Richardsen},
  title = 	 {Lipid vesicles and membrane fusion},
  journal = 	 {Adv. Drug. Deliv.},
  year = 	 {1999},
  volume = 	 {38},
  pages = 	 {207-232}
}

@Article{Chanturiya97,
  author = 	 {A. Chanturiya and L.V. Chernomordik and J. Zimmerberg},
  title = 	 {Flickering fusion pores comparable with initial exocytotic pores occur in protein-free phospholipid bilayers},
  journal = 	 {Proc. Natl. Acad. Sci. USA},
  year = 	 {1997},
  volume = 	 {94},
  pages = 	 {14423-14428}
}


@Article{Chen97,
  author =       {Z. Chen and R. P. Rand},
  title =        {The influence of cholesterol on phospholipid membrane
                  curvature and bending elasticity},
  journal =      {Biophys. J.},
  year =         {1997},
  volume =       {73},
  pages =        {267-276}
}

@Article{Chen01,
  author =       {Y. A. Chen and R. H. Scheller},
  title =        {SNARE-mediated membrane fusion.},
  journal =      {Nat. Rev. Mol. Cell. Biol.},
  year =         {2001},
  volume =       {2},
  pages =        {98-106}
}

@Article{Chernomordik95,
  author = 	 {L. Chernomordik and M.M. Kozlov and J. Zimmerberg},
  title = 	 {Lipids in biological membrane fusion},
  journal = 	 {J. Membr. Biol.},
  year = 	 {1995},
  volume = 	 {146},
  pages = 	 {1-14}
}


@Article{Chernomordik96,
  author = 	 {L. Chernomordik},
  title = 	 {Non-bilayer lipids and biological  fusion intermediates},
  journal = 	 {Chem. and Phys. Lipids},
  year = 	 {1996},
  volume = 	 {81},
  pages = 	 {203-213}
}


@Article{Chernomordik85,
  author = 	 {L. V. Chernomordik and M. M. Kozlov and G. B. Melikyan and I. G. Abidor and V. S. Markin and Yu. A. Chizmadzhev},
  title = 	 {The shape of lipid molecules and monolayer membrane fusion},
  journal = 	 {Biochim. Biophys. Acta},
  year = 	 {1985},
  volume = 	 {812},
  pages = 	 {643-655}
}

@Article{Chernomordik03,
  author = 	 {L. V. Chernomordik and M. M. Kozlov},
  title = 	 {Protein-lipid interplay in fusion and fission of biological membranes},
  journal = 	 {Annu. Rev. Biochem},
  year = 	 {2003},
  volume = 	 {72},
  pages = 	 {175-207}
}

@Article{Cohen04,
  author = {F. S. Cohen and G. B. Melikyan},  
  title  = {The energetics of membrane fusion from binding, through hemifusion, pore formation, and pore enlargement},
  journal = {J.  Membrane Biol.},
  year = {2004},
  volume = {199},
  pages = {1-14} 
}
 
@Book{Davis,
 author ={H.T. Davis},
 title  ={Statistical mechanics of phases, interfaces, and thin films},
 publisher ={Wiley-VCH},
 year ={1996},
 address={New York, NY}
}

@Article{DeKruijff97,
  author = 	 {B. de Kruijff},
  title = 	 {Lipid polymorphism and biomembrane function},
  journal = 	 {Curr. Opin. Chem. Biol.},
  year = 	 {1997},
  volume = 	 {1},
  pages = 	 {564-569}
}


@Article{Devaux91,
   author = {P.F. Devaux},
   title = {Static and dynamic lipid asymmetry in cell membranes},
   journal = {Biochemistry},
   year = {1991},
   volume = {30},
   pages = {1163-1173}
}


@Article{discher99,
  author = 	 {B. D. Discher and Y-Y. Won and D. S. Ege and J. C-M. Lee and F. S. Bates and D. E. Discher and D. A. Hammer},
  title = 	 {Polymersomes: tough vesicles made from diblock copolymers},
  journal = 	 {Science},
  year = 	 {1999},
  volume = 	 {284},
  pages = 	 {1143-1146}
}

@Article{Disko93,
  author = 	 {M. M. Disko and K. S. Liang and S. K. Behal and R. J. Roe and K. J. Jeon},
  title = 	 {Catenoid-lamellar phase in blends of styrene-butadiene diblock copolymer and homopolymer},
  journal = 	 {Macromolecules},
  year = 	 {1993},
  volume = 	 {26},
  pages = 	 {2983-2986}
}


@Article{Drolet99,
 author =         {F. Drolet and G.H. Fredrickson},
 title = {Combinatorial screening of complex block copolymer assembly with 
          self-consistent field theory},
 journal = {Phys. Rev. Lett.},
 year = {1999},
 volume = {83},
 pages = {4317-4320}
}

 
@Article{Dunina00,
  author = 	 {A. Ya. Dunina-Barkovskaya and A. V. Samsonov and V. S. 
                  Pivovarov and V. A. Frolov},
  title = 	 {Hemagglutinin-induced fusion of HAb2 and PLC cells:  
                  dynamics of fusion pore conductance},
  journal = 	 {Membr. Cell Biol.},
  year = 	 {2000},
  volume = 	 {13},
  pages = 	 {567-580}
}

@Article{Duque03,
 author ={Daniel Duque},
 title = {Theory of copolymer micellization},
 journal = {J. Chem. Phys.},
 year = {2003},
 volume = {119},
pages = {5701-5704}
}

@Article{Eastman92,
  author = {S.J. Eastman and M. J. Hope and K.F. Wong and P. R. Cullis},
  title = {Influence of phospholipid asymmetry on fusion between 
           large unilamellar vesicles},
  journal = {Biochemistry},
  year = {1992},
  volume = {31},
  pages = {4262-4268}
} 

@Article{Evans02,
  author = 	 {K. O. Evans and B. R. Lentz},
  title = 	 {Kinetics of lipid rearrangements during poly(ethylene glycol)-mediated fusion of highly curved unilamellar vesicles},
  journal = 	 {Biochemistry},
  year = 	 {2002},
  volume = 	 {41},
  pages = 	 {1241-1249}
}

@Article{Fernandez84,
  author = 	 {J.M. Fernandez and E. Neher and B.D. Gomperts},
  title = 	 {Capacitance measurements reveal stepwise fusion events in degranulating mast cells},
  journal = 	 {Nature},
  year = 	 {1984},
  volume = 	 {312},
  pages = 	 {453-455}
}


@Book{Flint00,
  author = {S.J. Flint and V.R. Racaniello and L.W. Enquist and A.M Skalka and R.M. Krug},
  title ={Virology: Molecular biology, pathogenesis, and control},
  publisher = {ASM Press},
  year = {2000},
  address = {Washington, D.C.},  
  note ={p. 136}
}


@Article{Frolov03,
  author = 	 {V. A. Frolov and A. Ya. Dunina-Barkovskaya and 
A. V. Samsonov and J. Zimmerberg
},
  title = 	 {Membrane permeability changes at early stages of influenza hemagglutinin-mediated fusion},
  journal = 	 {Biophys. J.},
  year = 	 {2003},
  volume = 	 {85},
  pages = 	 {1725-1733}
}

@Article{Gotzelmann98,
  author   =     {B. G{\"o}tzelmann and R. Evans and S. Dietrich},
  title    =     {Depletion forces in fluids},
  journal  =     {Phys. Rev. E},
  year     =     {1998},
  volume   =     {57},
  pages    =      {6785-6800}
}


@Article{Groot01,
  author = 	 {R.D. Groot and K.L. Rabone},
  title = 	 {Mesoscopic simulation of cell membrane damage, 
                 morphology change and rupture by nonionic surfactants},
  journal = 	 {Biophys. J.},
  year = 	 {2001},
  volume = 	 {81},
  pages = 	 {725-736}
}

@Article{Gruner83,
  author = { S. M. Gruner},
  title = {Stability of lyotropic phases with curved interfaces},
  journal = {J. Phys. Chem.},
  year = {1989},
  volume = { 93},
  pages = {7562-1570}
}

@Article{Haque02,
  author = 	 {Md. E. Haque and B. R. Lentz},
  title = 	 {Influence of gp41 fusion peptide on the kinetics of poly(ethylene glycol)-mediated model membrane fusion},
  journal = 	 {Biochemistry},
  year = 	 {2002},
  volume = 	 {41},
  pages = 	 {10866-10876}
}

@Article{Hope80,
  author = {M. J. Hope and P. R. Cullis},
  title = {Effects of divalent cations and $pH$ on phosphatidylserine model membranes: A $^{31}$P NMR study},
  journal = { Biochem. and Biophys. Res. Comm.},
  year = {1980},
  volume = {92},
  pages = {846-852}
}


@Article{Hope83,
 author = {M. J.  Hope and D. C, Walker and P.R. Cullis},
 title = {Ca$^{2+}$ and $pH$ induced fusion of small unilamellar vesicles consisting of
 phosphatidylethanomaline and negatively charged phospholipids: a freeze 
 fracture study},
 journal = {Biochem. Biophys. Res. Commun.},
 year = {1983},
 volume = {110},
 pages =  {15-22}
 } 

@Article{Jahn02,
  author = 	 {R. Jahn and H. Grubm{\"u}ller},
  title = 	 {Membrane fusion},
  journal = 	 {Curr. Opinion in Cell Biol.},
  year = 	 {2002},
  volume = 	 {14},
  pages = 	 {488-495}
}

@Article{Kanaseki97,
  author = 	 {T. Kaneseki and K. Kawasaki and M. Murata and Y. Ikeuchi and S-i. Ohnishi},
  title = 	 {Structural features of membrane fusion between influenza virus and liposome revealed by quick-freezing electron microscopy},
  journal = 	 {J. Cell Biol.},
  year = 	 {1997},
  volume = 	 {137},
  pages = 	 {1041-1056}
}

@Article{Kasson04,
  author = 	 {P.M. Kasson and V. S. Pande},
  title = 	 {Molecular dynamics simulation of lipid reorientation at 
                  bilayer edges},
  journal = 	 {Biophys. J},
  year = 	 {2004},
  volume = 	 {86},
  pages = 	 {3744-3749}
}



@article{Katsov04,
  author =       {K. Katsov and M. M{\"u}ller and M. Schick},
  title =        {Field theoretic study of bilayer membrane fusion: I. Hemifusion mechanism},
  journal =      {Biophys. J.},
  year =         {2004},
  volume =       {87},
  pages =        {3277-3290}
}  

@article{Katsov06,
  author =       {K. Katsov and M. M{\"u}ller and M. Schick},
  title =        {Field theoretic study of bilayer membrane fusion: II. 
Mechanism of a stalk-hole complex},
  journal =      {Biophys. J.},
  year =         {2006},
  volume =       {90},
  pages =        {915-926}
}  

@Article{Kozlov83,
  author = 	 {M. M. Kozlov and V. S. Markin},
  title = 	 {Possible mechanism of membrane fusion},
  journal = 	 {Biofizika},
  year = 	 {1983},
  volume = 	 {28},
  pages = 	 {255-261}
}


@Article{Kozlov98,
   author =      {M.M. Kozlov and L.V. Chernomordik},
   title =       {A mechanism of protein-mediated fusion: coupling between 
                 refolding of the influenza hemagglutinin and lipid 
                 rearrangements},
   journal =     {Biophys. J.},
   year =        {1998},
   volume =      {75},
   pages =       {1384-1396}
} 

  
@Article{Kozlovsky02,
  author = 	 {Y. Kozlovsky and M. M. Kozlov},
  title = 	 {Stalk model of membrane fusion: solution of energy crisis},
  journal = 	 {Biophys. J.},
  year = 	 {2002},
  volume = 	 {82},
  pages = 	 {882-895}
}

@Article{Kozlovsky002,
author = 	 {Y. Kozlovsky and L. V. Chernomordik and M. M. Kozlov},
  title = 	 {Lipid intermediates in membrane fusion: formation, structure, and decay of hemifusion diaphragm},
  journal = 	 {Biophys. J.},
  year = 	 {2002},
  volume = 	 {83},
  pages = 	 {2634-2651}
}

@Article{Kuzmin01,
  author = 	 {P. I. Kuzmin and J. Zimmerberg and Yu. A. Chizmadzhev and F. S. Cohen},
  title = 	 {A quantitative model for membrane fusion based on low-energy intermediates},
  journal = 	 {Proc. Natl. Acad. Sci. U.S.A.},
  year = 	 {2001},
  volume = 	 {98},
  pages = 	 {7235-7240}
}

@Article{Lee97,
  author = 	 {J. Lee and B. R. Lentz},
  title = 	 {Evolution of lipidic structures during model membrane fusion and the relation of this process to cell membrane fusion},
  journal = 	 {Biochemistry},
  year = 	 {1997},
  volume = 	 {36},
  pages = 	 {6251-6259}
}

@Article{Lee98,
  author = 	 {J. Lee and B. R. Lentz},
  title = 	 {Secretory and viral fusion may share mechanistic events with fusion between curved lipid bilayers},
  journal = 	 {Proc. Natl. Acad. Sci. USA},
  year = 	 {1998},
  volume = 	 {95},
  pages = 	 {9274-9279}
}

@Article{Leikin96,
  author =       {S. Leikin and M. M. Kozlov and N. L. Fuller and R. P. Rand},
  title =        {Measured effects of dyacilglycerol on structural and elastic properties of phospholipid membrane},
  journal =      {Biophys. J.},
  year =         {1996},
  volume =       {71},
  pages =        {2623-2632}
}


@Article{Lentz97,
  author = 	 {B. R. Lentz and W. Talbot and J. Lee and L.-X. Zheng},
  title = 	 {Transbilayer lipid redistribution accompanies poly(ethylene glycol) treatment of model membranes but is not induced by fusion},
  journal = 	 {Biochemistry},
  year = 	 {1997},
  volume = 	 {36},
  pages = 	 {2076-2083}
}

@Article{Lentz00,
  author = 	 {B. R. Lentz and  V. Malinin and Md. E. Haque and K. Evans},
  title = 	 {Protein machines and lipid assemblies: current views of cellmembrane fusion},
  journal = 	 {Curr. Opinion in Struct. Biol.},
  year = 	 {2000},
  volume = 	 {10},
  pages = 	 {607-615}
}

@Article{Lentz06,
   author={B.R. Lentz},
   title ={Seeing is believing: The stalk intermediate},
   journal={Biophys. J.},
   year={2006},
   volume={91},
   pages={??}
   }

@Article{Li00,
  author = 	 {X.-J. Li and M. Schick},
  title = 	 {Distribution of lipids in nonlamellar phases of their mixtures},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2000},
  volume = 	 {112},
  pages = 	 {6063-6072}
}

@Article{Leontiadou04,
  author = 	 {H. Leontiadou and A.E. Mark and S.J. Marrink},
  title = 	 {Molecular dynamics simulations of hydrophilic pores in lipid bilayers},
  journal = 	 {Biophys. J.},
  year = 	 {2004},
  volume = 	 {86},
  pages = 	 {2156-2164}
}

@Article{Loison04,
  author = 	 {C. Loison and M. Mareschal and F. Schmid},
  title = 	 {Pores in bilayer membranes of amphiphilic molecules: Coarse-grained molecular dynamics simulations compared with simple mesoscopic models},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2004},
  volume = 	 {121},
  pages = 	 {1890-1900}
}

@Article{Malinin04,
  author = 	 {V. S. Malinin and B. R. Lentz},
  title = 	 {Energetics of vesicle fusion intermediates: Comparison of calculations with observed effects of osmotic and curvature stresses},
  journal = 	 {Biophys. J.},
  year = 	 {2004},
  volume = 	 {86},
  pages = 	 {2951-2964}
}


@Article{Markin02,
  author = 	 {V. S. Markin and J. P. Albanesi},
  title = 	 {Membrane fusion: stalk model revisted},
  journal = 	 {Biophys. J.},
  year = 	 {2002},
  volume = 	 {82},
  pages = 	 {693-712}
}

@Article{Markin83,
  author = 	 {V. S. Markin and M. M. Kozlov},
  title = 	 {Primary act in the process of membrane fusion},
  journal = 	 {Biofizika},
  year = 	 {1983},
  volume = 	 {28},
  pages = 	 {73-78}
}

@Article{Marrink03,
  author =       {Siewart J. Marrink and Alan E. Mark},
  title =         {The mechanism of vesicle fusion as revealed by molecular 
                   dynamics simulations},
  journal =         {J. Am. Chem. Soc.},
  year   =        {2003},
  volume =        {125},
  pages  =         {11144-11145}
}


@Article{Matsen95,
  author = 	 {M. W. Matsen},
  title = 	 {Phase Behavior of Block Copolymer/Homopolymer Blends},
  journal = 	 {Macromolecules},
  year = 	 {1995},
  volume = 	 {28},
  pages = 	 {5765-5773}
}

@Article{Matsen96,
  author = 	 {M. W. Matsen and F. S. Bates},
  title = 	 {Origins of complex self-assembly in block copolymers},
  journal = 	 {Macromolecules},
  year = 	 {1996},
  volume = 	 {29},
  pages = 	 {7641-7644}
}

@Article{Matsen97,
  author = 	 {M. W. Matsen},
  title = 	 {Thin films of block copolymer},
  journal = 	 {J. Chem. Phys.},
  year = 	 {1997},
  volume = 	 {106},
  pages = 	 {7781-7791}
}



@Article{Matsen94,
  author = 	 {M. W. Matsen and M. Schick},
  title = 	 {Stable and Unstable phases of a diblock copolymer melt},
  journal = 	 {Phys. Rev. Lett.},
  year = 	 {1994},
  volume = 	 {72},
  pages = 	 {2660-2663}
}


@Article{Matsen99,
  author = 	 {M. W. Matsen},
  title = 	 {Elastic properties of a diblock copolymer monolayer and their relevance to bicontinuous microemulsion},
  journal = 	 {J. Chem. Phys},
  year = 	 {1999},
  volume = 	 {110},
  pages = 	 {4658-4667}
}

@Article{Mayer02,
  author = 	 {A. Mayer},
  title = 	 {Membrane fusion in eukaryotic cells},
  journal = 	 {Ann. Rev. Cell and Dev. Biol.},
  year = 	 {2002},
  volume = 	 {18},
  pages = 	 {289-315}
}

@Article{Melikov01,
  author  =      {K. C. Melikov and V.A. Frolov and A Shcherbakov and A. V. Samsonov and Y. A. Chizmadzhev and L. V. Chernomordik},
  title   =      {Voltage-induced nonconductive pre-pores and metastable single pores in unmodified planar lipid bilayer.},
  journal =      {Biophys. J.},
  year =         {2001},
  volume =       {80},
  pages =        {1829-1836}
}


@Article{Melikyan95,
  author = 	 {G. B. Melikyan and J. M. White and F. S. Cohen},
  title = 	 {GPI-anchored influenza hemagglutinin induces hemifusion to both red blood cells and planar bilayer membranes},
  journal = 	 {J. Cell Biol.},
  year = 	 {1995},
  volume = 	 {131},
  pages = 	 {679-691}
}

@Article{Monck90,
  author = 	 {J. R. Monck and G.A. de Toledo and J. M. Fernandez},
  title = 	 {Tension in granule secretory membranes causes extensive membrane transfer through the exocytotic fusion pore},
  journal = 	 {Proc. Natl. Acad. Sci.USA},
  year = 	 {1990},
  volume = 	 {87},
  pages = 	 {7804-7808}
}


@Article{Monck96,
  author = 	 {J. R. Monck and J. M. Fernandez},
  title = 	 {The fusion pore and mechanisms of biological membrane fusion},
  journal = 	 {Curr. Opin. Cell Biol.},
  year = 	 {1996},
  volume = 	 {8},
  pages = 	 {524-533}
}


@Article{Morein96,
  author  =     {S. Morein and A. Andersson and L. Rilfors and G. Lindblom},
  title   =     {Wild-type escherichia coli cells regulate the  membrane lipid composition in a window between gel and non-lamellar structures}, 
  journal =      {J. Biol. Chem.},
  year =         {1996},
  volume  =      {271},
  pages   =      {6801-6809}
}


@Article{Moroz97,
  author = 	 {J. D. Moroz and P. Nelson},
  title = 	 {Dynamically-stabilized pores in bilayer membranes},
  journal = 	 {Biophys. J.},
  year = 	 {1997},
  volume = 	 {72},
  pages = 	 {2211-2216}
}


@Article{Mueller02,
  author = 	 {M. M\"uller and  K. Katsov and M. Schick},
  title = 	 {New mechanism of membrane fusion},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2002},
  volume = 	 {116},
  pages = 	 {2342-2345}
}

@Article{Mueller002,
  author = 	 {M. M\"uller and  G. Gompper},
  title = 	 {Elastic properties of polymer interfaces: 
Aggregation of pure diblock, mixed diblock, and triblock copolymers},
  journal = 	 {Phys.Rev. E},
  year = 	 {2002},
  volume = 	 {66},
  pages = 	 {041805,1-041805,13}
}

@Article{Mueller0002,
  author = 	 {M. M\"uller and L.G. Mac Dowell and P. Virnau and K. Binder},
  title = 	 {Interface properties and bubble nucleation in compressible 
mixtures containing polymers},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2002},
  volume = 	 {117},
  pages = 	 {5480-5496}
}

@Article{Mueller03,
  author =       {M. M\"uller and  K. Katsov and M. Schick},
  title  =       {A new mechanism of model membrane fusion determined from Monte Carlo simulation},
  journal =       {Biophys. J.},
  year =          {2003},
  volume =        {85},
  pages =          {1611-1623}
}


@Article{Mueller003,
  author =       {M. M\"uller and  K. Katsov and M. Schick},
  title  =       {Coarse-grained models and collective phenomena in membranes:computer simulation of membrane fusion},
  journal =       {Journal of polymer science; Part B: Polymer physics},
  year =          {2003},
  volume =        {41},
  pages =          {1441-1450}
}


@Article{Mueller96,
  author = 	 {M. M\"uller and M. Schick},
  title = 	 {Structure and nucleation of pores in polymeric bilayers: a Monte Carlo simulation},
  journal = 	 {J. Chem. Phys.},
  year = 	 {1996},
  volume = 	 {105},
  pages = 	 {8282-8292}
}

@Article{Netz97,
  author = 	 {R.R. Netz and D. Andelman and M. Schick},
  title = 	 {Interfaces of modulated phases},
  journal = 	 {Phys. Rev. Lett.},
  year = 	 {1997},
  volume = 	 {79},
  pages = 	 {1058-1061}
}


@Article{Niles90,
  author =        {W.D. Niles and M.E. Peeples and F.S. Cohen},
  title =         {Kinetics of virus-induced hemolysis measured for single 
erythrocytes},
  journal =      {Virology},
  year =         {1990},
  volume =       {174},
  pages =        {593-598}
} 

@Article{Noguchi01,
  author = 	 {H. Noguchi and M. Takasu},
  title = 	 {Fusion pathways of vesicles: A Brownian dynamics simulation},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2001},
  volume = 	 {115},
  pages = 	 {9547-9551}
}


@Article{Parsegian95,
  author = 	 {V. Parsegian and R. Rand},
  title = 	 {Interaction on membrane assemblies. In Lipowsky, R. and Sackmann, E. editors},
  journal = 	 {Structure and Dynamics in Membranes, volume 1B of Handbook of Biological Physics},
  year = 	 {1994},
  volume ={},
  pages  =        {643-690. Elsevier Science B.V.}
}

@Article{Peliti85,
  author = {L. Peliti and S. Leibler},
  title  = {Effects of thermal fluctuations on systems with small surface 
            tensions},
  journal = {Phys. Rev. Lett.},
  year    = {1985},
  volume  = {54},
  pages   = {1690-1693}
}

@Article{Rand89,
  author = 	 {R. P. Rand and V. A. Parsegian},
  title = 	 {Hydration forces between phospholipid bilayers},
  journal = 	 {Biochim. Biophys. Acta},
  year = 	 {1989},
  volume = 	 {988},
  pages = 	 {351-376}
}

@Article{Rand90,
  author = 	 {R. P. Rand and N. L. Fuller and S. M. Gruner and V. A. Parsegian},
  title = 	 {Membrane curvature, lipid segregation, and structural transitions for phospholipids under dual-solvent stress},
  journal = 	 {Biochemistry},
  year = 	 {1990},
  volume = 	 {29},
  pages = 	 {76-87}
}

@Article{Rasmussen02,
 author = {K.O. Rasmussen and G. Kalosakas},
 title = {Improved numerical algorithm for exploring block copolymer mesophases},
 journal = {J. Polym. Sci. Pol. Phys.},
 year = {2002},
 volume ={40},
 pages ={1777-1783}
} 

@Article{Rothman77,
  author = {J. E. Rothman and J. Lenard},
  title = {Membrane Asymmetry},
  journal = {Science},
  year = {1977},
  volume = {195},
  pages = {743-753}
}


@Book{Safran94,
  author = 	 {S. A. Safran},
  title = 	 {Statistical thermodynamics of surfaces, interfaces and membranes},
  publisher = 	 {Addison Wesley},
  year = 	 {1994},
  address = {Reading MA}
}

@Article{Schmid98,
  author = 	 {F. Schmid},
  title = 	 {Self-consistent field theories for complex fluids},
  journal = 	 {J. Phys-condensmat},
  year = 	 {1998},
  volume = 	 {10},
  pages = 	 {8105-8138}
}

@Article{Seigneuret84,
   author = {M. Seigneuret and P. F. Devaux},
   title = {Asymmetric distribution of spin-labeled 
           phospholipids in the erythrocyte membrane: Relation to shape changes},
   journal = {Proc. Natl Acad.  Sci. USA},
   year = { 1984},
   volume = {81}, 
   pages = {3751-3755}
}
 

@Article{Siegel86,
  author = 	 {D. P. Siegel},
  title = 	 {Inverted micellar intermediates and the transitions between lamellar, inverted hexagonal, and cubic lipid phases. II. Implications for 
membrane-membrane interactions and membrane fusion.},
  journal = 	 {Biophys. J.},
  year = 	 {1986},
  volume = 	 {49},
  pages = 	 {1171-1183}
}

@Article{Siegel93,
  author = 	 {D. P. Siegel},
  title = 	 {Energetics of intermediates in membrane fusion:comparison of stalk and inverted micellar intermediate mechanisms},
  journal = 	 {Biophys. J.},
  year = 	 {1993},
  volume = 	 {65},
  pages = 	 {2124-2140}
}

@Article{Shangguan96,
  author = 	 {T. Shangguan and D. Alford and J. Bentz},
  title = 	 {Influenza virus-liposome lipid mixing is leaky and largely insensitive to the material properties of the target membrans},
  journal = 	 {Biochemistry},
  year = 	 {1996},
  volume = 	 {25},
  pages = 	 {4956-4965}
}

@Article{Shelley,
   author = {J. C. Shelley and M.Y. Shelley and R.C. Reeder and S. Bandyopadhay and M.L. Klein},
   title = {A coarse grain model for phospholipid simulations},
   journal = {J. Phys. Chem. B},
   year = {2001},
   volume = {105},
   pages = {4464-4470}
}

@Article{Shillcock02,
  author = 	 {J. C. Shillcock and R. Lipowsky},
  title = 	 {Equilibrium structure and lateral stress distribution of amphiphilic bilayers from dissipative particle dynamics simulations},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2002},
  volume = 	 {117},
  pages = 	 {5048-5061}
}

@Article{Skehel00,
  author = 	 {J.J. Skehel and D.C. Wiley},
  title = 	 {Receptor binding and membrane fusion in virus entry: The influenza hemagglutinin},
  journal = 	 {Annu. Rev. Biochem.},
  year = 	 {2000},
  volume = 	 {69},
  pages = 	 {531-569}
}

@Article{Smeijers06,
  author = {A. F. Smeijers and A. J. Marvoort and K. Pieterse and P. A. J. Hilbers},
  title = {A detailed look at vesicle fusion},
  journal = { J. Phys. Chem. B},
  year = {2006},
  volume = {110},
  pages = { 13212-13219}
}   


@Article{Smit02,
  author = 	 {J. M. Smit and G. Li and P. Schoen and J. Corver and R. Bittman and K.-C. Lin and J. Wilschut},
  title = 	 {Fusion of alphaviruses with liposomes is a non-leaky process},
  journal = 	 {FEBS Lett.},
  year = 	 {2002},
  volume = 	 {421},
  pages = 	 {62-66}
}

@Article{Spruce90,
 author =         {A.E. Spruce and L.J. Breckenridge and A. K. Lee and W. Almers},
 title  =         {Properties of the fusion pore that forms during exocytosis of a mast cell secretory vesicle},
 journal =        {Neuron},
 year =           {1990},
 volume =         {4},
 pages =          {643-654}
}

@Article{Spruce91,
 author =         {A.E. Spruce and A. Iwata and W. Almers},
 title  =         {The first milliseconds of the pore formed by a fusogenic viral envelope protein during membrane fusion},
 journal =        {Proc Natl Acad Sci U S A},
 year =           {1991},
 volume =         {88},
 pages =          {3623-3627}
}

@Article{Stevens03,
  author =       {Mark J. Stevens and Jan Hoh and Thomas Woolf},
  title  =        {Insights into the molecular mechanism of membrane fusion 
                  from simulation: evidence for the association of splayed 
                  tails},
  journal =       {Phys. Rev. Lett.},
  year =          {2003},
  volume =         {91},
  pages =          {188102-1-188102-4}
}

@Article{Tamm03,
  author = 	 {L.K. Tamm and J. Crane and V. Kiessling},
  title = 	 {Membrane fusion: a structural perspective on the interplay of lipids and proteins},
  journal = 	 {Curr. Opin. Struct. Biol.},
  year = 	 {2003},
  volume = 	 {13},
  pages = 	 {453-466}
}


@Article{Thompson00,
   author =       {R. Thompson and M. Matsen},
   title  =       {Effective interaction between monolayers of block copolymer compatibilizer in a polymer blend},
   journal =      {J. Chem. Phys.},
   year    =      {2000},
   volume  =       {112},
   pages   =       {6863-6872}
} 

@Article{Tieleman03,
  author = 	 {D.P. Tieleman and H. Leontiadou and A.E. Mark and S.J. Marrink},
  title = 	 {Simulation of pore formation in lipid bilayers by mechanical stress and electric fields},
  journal = 	 {J. Am. Chem. Soc.},
  year = 	 {2003},
  volume = 	 {125},
  pages = 	 {6382-6383}
}

@Article{Tolpekina04,
  author = 	 {T.V. Tolpekina and W.K. den Otter and W.J. Briels},
  title = 	 {Simulations of stable pores in membranes: System size dependence and line tension},
  journal = 	 {J. Chem. Phys.},
  year = 	 {2004},
  volume = 	 {121},
  pages = 	 {8014-8020}
}


@Article{Tse93,
 author =        {F.W. Tse and A. Iwata and W. Almers},
 title  =        {Mebrane flux through the pore formed by a fusogenic viral envelope protein during cell fusion},
 journal =       {J. Cell Biol.},
 year =          {1993},
 volume =        {121},
 pages =         {543-552}
}

@Article{Weislander97,
  author  =        {\AA Wieslander and Olf P. Karlsson},
  title   =        {Regulation of lipid synthesis in Acholeplasma laidlawii},
  journal =        {Current Topics in Membranes},
  year    =        {1997},
  volume  =        {44},
  pages   =         {517-540}
}



@Article{Yang02,
  author = 	 {L. Yang and H. W. Huang},
  title = 	 {Observation of a membrane fusion intermediate structure},
  journal = 	 {Science},
  year = 	 {2002},
  volume = 	 {297},
  pages = 	 {1877-1879}
}

@Article{Zhelev93,
  author = 	 {D.V. Zhelev and D. Needham},
  title = 	 {Tension-stabilized pores in giant vesicles-determination of pore-saize and pore line tension},
  journal = 	 {Biochim. Biophys. Acta},
  year = 	 {1993},
  volume = 	 {1147},
  pages = 	 {89-104}
}


@Article{Zimmerberg99,
  author = 	 {J. Zimmerberg and L. V. Chernomordik},
  title = 	 {Membrane fusion},
  journal = 	 {Adv. Drug Deliv. Rev.},
  year = 	 {1999},
  volume = 	 {38},
  pages = 	 {197-205}
}





